Wafer-scale Computing: Advancements, Challenges, and Future Perspectives

Nowadays, artificial intelligence (AI) technology with large models plays an increasingly important role in both academia and industry. It also brings a rapidly increasing demand for the computing power of the hardware. As the computing demand for AI continues to grow, the growth of hardware computing power has failed to keep up. This has become a significant factor restricting the development of AI. The augmentation of hardware computing power is mainly propelled by the escalation of transistor density and chip area. However, the former is impeded by the termination of the Moore's Law and Dennard scaling, and the latter is significantly restricted by the challenge of disrupting the legacy fabrication equipment and process. In recent years, advanced packaging technologies that have gradually matured are increasingly used to implement bigger chips that integrate multiple chiplets, while still providing interconnections with chip-level density and bandwidth. Compared to conventional high-performance computing paradigms such as multi-accelerator and datacenter-scale computing, Wafer-scale Computing shows remarkable advantages in communication bandwidth, integration density, and programmability potential. Not surprisingly, disruptive Wafer-scale Computing also brings unprecedented design challenges for hardware architecture, design-system-technology co-optimization, power and cooling systems, and compiler tool chain. At present, there are no comprehensive surveys summarizing the current state and design insights of Wafer-scale Computing. This paper aims to take the first step to help academia and industry review existing wafer-scale chips and essential technologies in a one-stop manner. So that people can conveniently grasp the basic knowledge and key points, understand the achievements and shortcomings of existing research, and contribute to this promising research direction.

==> data/interconnection-old.tex <==
% !TeX root = ../bare_jrnl_new_sample4.tex

\section{Interconnect Interfaces and Protocols \label{secInterconnect}}

TODO: Discuss with Xingmao
%TODO：内部？外部？

The interconnect interface and protocol design between dies are extremely critical to the performance of wafer-scale chips. Compared with traditional chips, interconnect the design of interface and protocol of dies not only need to consider the unit transmission bandwidth, power consumption per bit, etc., but also need to consider the requirements of advanced manufacturing process, packaging technology and system integration. Generally, in order to achieve high-speed and efficient communication between dies, the optimal interconnection scheme must need trade-off between various indicators and constraints according to the actual application requirements, so as to meet the requirements of efficient interconnection and communication of dies.


\subsection{Internal Interconnect Interface}
\subsubsection{Apple UltraFusion}

Apple’s M1 Ultra chip \cite{mattioli2022meet} uses TSMC's 5nm process. It includes 20 CPU cores, 64 GPU cores, 32 neural network engine NPU cores, 128GB of memory, and 800GBps of memory bandwidth. It also solves the interconnection of very-large area Chiplets.

Especially, the UltraFusion interconnect technology design of die-to-die is extremely impressive. According to the current published papers and patents, UltraFusion should be an interconnect architecture based on TSMC’s CoWoS-S5 Interconnect technology, using Silicon Interposer and Micro-Bump technology. UltraFusion also provides more than 10,000 die-to-die connection signal lines, with an ultra-high interconnection bandwidth of 2.5TB/s. Compared to other multi-chip module (MCM) packaging technologies, UltraFusion's interposer provides dense and short metal interconnects between logic dies or between logic dies and memory stacks. It has better inter-chip integrity, lower power consumption, and can run at higher clock frequencies.

In addition, UltraFusion effectively improves packaging yield and reduces costs through Die-Stitching technology. In UltraFusion, only the Known Good Die (KGD) is bonded, which avoids the problem that the failed chips in traditional Wafer on Wafer (WoW) or Chip on Wafer (CoW) are encapsulated, thereby increasing post-package yield and reducing overall average cost.


\subsubsection{Intel AIB/MDIO}
Intel’s AIB/MDIO [2] provides a parallel interconnection standard for the physical layer. MDIO technology provides higher transmission efficiency, and its response speed and bandwidth density are more than twice that of AIB. AIB and MDIO are applied to advanced 2.5D/3D packaging technologies with short interconnect communication distance and high interconnect density, such as EMIB [3] and Foveros [4].


\subsubsection{Intel PCIe gen 4, 5, and 6}
PCI express (PCI-e) is a general-purpose serial interconnect technology that is not only suitable for interconnecting GPUs, network adapters, and other additional devices, but also for die-to-die interconnect communication.

Since PCI-e Gen 3 was widely adopted, it has been developing rapidly. The transfer rate of PCI-e Gen 4 is 16 GT/s, and the theoretical throughput is 32 GB/s for 16x ports. PCI-e Gen 5, which was finalized in 2019, has twice the transfer rate of Gen 4 at 32GT/s, and the 16x port has a bandwidth of about 64GB/s. Currently, the latest PCI-e Gen 6 standard has now been released, which doubles the data transfer rate from 32GT/s to 64GT/s, providing approximately 128 GB /s of bandwidth for 16x ports. In addition, the PCI-e Gen 6 uses a new PAM4 encoding to replace the PCIe 5.0 NRZ, using a 1b/1b encoding scheme, which can encapsulate more data in a single channel in the same time. The PCIe 6.0 also introduces low-latency forward error correction (FEC) and related mechanisms to improve bandwidth efficiency and reliability.

\subsubsection{Intel CXL}
Compute Express Link (CXL) is an open standard for high-speed interconnects designed to address the interconnection gap between CPUs and devices and between CPUs and memory. Intel pointed out that PCIe is perfect for client machines without too many devices and too much memory, but when dealing with multiple devices that require bandwidth and huge shared memory pools, PCIe has huge delays and inefficient access mechanisms. 

CXL is designed to overcome these problems without giving up the best parts of PCIe - the simplicity and adaptability of its physical layer. CXL is based on the physical layer of PCI-e Gen 5 and uses the same physical and electrical interface. CXL provides protocols in three areas: CXL.io, CXL.cache, and CXL.memory. CXL.io is the simplest one, which is very similar to PCI-e, supporting the same features as PCI-e; CXL.cache is used to handle device access to local processor memory, for example, to allow network drives to access their own caches; CXL.memory is used to provide processor access to attached device memory (non-native memory).

\subsubsection{Intel UCIe 1.0}
Intel, AMD, Arm, Qualcomm, TSMC and other industry giants jointly established the Chiplet Standard Alliance and officially launched the universal Chiplet high-speed interconnect standard "Universal Chiplet Interconnect Express" (Universal Chiplet Interconnect Express, UCIe), aiming to define an open, interoperable chiplet ecosystem standard. The UCIe 1.0 protocol uniformly uses Intel's mature PCIe and CXL (Compute Express Link) interconnection bus technologies. PCIe provides broad interoperability and flexibility, while CXL can be used for more advanced low-latency/high-throughput connections. The establishment of the UCIe standard maximizes the combination of the advantages of various fabs and technology companies, which is more conducive to the development of integrated circuit interconnection technology.


\subsubsection{TSMC LIPINCON}

TSMC’s LIPINCON \cite{lin20207} developed a high-performance parallel interconnect interface technology for the specific case of small chip memory interface. Through advanced packaging technology such as InFO and CoWoS, it can use simpler "clock forwarding" circuit, which greatly reduces the area overhead of the I/O circuit and its parasitic effects.

\subsubsection{NVIDA NVLink}
NVIDIA NVLink \cite{foley2017ultra} is the first high-speed inter-GPU interconnect technology to improve interconnect communication between GPUs in multi-GPU systems. NVLink allows multiple GPUs into a unified memory space, allowing one GPU to work on the local memory of another GPU that supports atomic operations. NVIDA P100 is the first product equipped with NVLink 1.0, and its single GPU has a bandwidth of 160GB/s, which is equivalent to 5 times the bandwidth of PCIe 4. The NVIDA V100 is equipped with NVLink 2.0, which increases the GPU bandwidth to 300G/s, which is almost 10 times that of PCIe 4. Currently, NVIDIA A100 integrates the latest NVLink 3.0. A single NVIDIA A100 Tensor core GPU supports up to 12 NVLink 3.0 connections, with a total bandwidth of 600G/s per second, almost 10 times the bandwidth of PCIe 5. In addition, NVIDIA has developed a separate NVLink switch chip - NVSwitch. NVSwitch has multiple ports, which can integrate multiple NVLinks and can be used to interconnect multiple GPUs. The NVSwitch 2.0 enables high-speed communication between all GPUs simultaneously at 600 GB/s.

\subsubsection{AMD Infinity Fabric}
Infinity Fabric (IF) \cite{beck2018zeppelin} is AMD's proprietary system interconnect, consisting of two systems, Infinity Scalable Data Fabric (SDF) and Infinity Scalable Control Fabric (SCF), which are responsible for data transmission and control respectively.  The IF can be used for interconnection of die to die or multiple GPUs.

\subsubsection{ARM CCIX}
Cache Coherent Interconnect for Accelerators (CCIX) [8] is an open standard interconnect designed to provide a cache coherent interconnect between CPUs and accelerators. CCIX mainly includes protocol specification and transport specification, which supports cache coherence by extending the functions of transaction layer and protocol layer on the standard PCIe data link layer. CCIX usually uses two mechanisms to improve performance and reduce latency. One is to use cache coherence to automatically keep the caches of processors and accelerators coherent. The other is to increase the raw bandwidth of the CCIX link, taking advantage of the standard 16 GT/s transfer rate of PCIe 4, up to a maximum rate of 25 GT/s.


\subsubsection{OCP ODSA BOW}
The BoW interface proposed by the OCP ODSA group focuses on solving the problem of parallel interconnections based on organic substrates. There are three types of BoW, namely BoW-base, BoW-fast and BoW-turbo. BoW-Base is designed for transmission distances less than 10mm, using an unterminated unidirectional interface with a data rate of up to 4Gbps per line. The BoW-Fast uses a termination interface for cable lengths up to 50mm. The transmission rate per line is 16Gbps. Compared with BoW-Fast, Bow-Turbo uses two wires and supports bidirectional 16Gbps transmission bandwidth.


\subsection{ External Interconnect Interface}
\subsubsection{Ethernet}
EtherNet/IP is an industrial communication network managed and published by the ODVA specification, which is realized by combining the CIP protocol, TCP/IP, and Ethernet. Currently, the mainstream Ethernet protocols include 100/25 Gigabit Ethernet, 200 and 400 Gigabit Ethernet, and RoCE. The 100/25 Gigabit Ethernet provides the ability to obtain a large number of 25 Gbps ports from a single switch using 100 Gbps switches and fanout cables. 200 Gbps Ethernet uses four 50 Gbps lanes per port, whereas the original 400 Gbps standard would use eight 50 Gbps lanes, simply doubling the number of lanes in a port. RoCE is a protocol for realizing RDMA access/transmission through conventional Ethernet. Its basic idea is to encapsulate an InfiniBand transmission packet into a normal Ethernet packet at the link layer. It uses Direct Memory Access (DMA), where the network adapter can read and write directly from host memory bypassing the CPU core, reducing CPU load.


\subsubsection{LR/MR/VSR SerDes}
For chip interconnection based on PCB boards, it can be divided into long reach/medium reach/very short reach SerDes according to transmission distance between chips. Although this interconnect technology has the advantages of high reliability, low cost and easy integration, it is difficult to meet the high-performance interconnect communication requirements between wafer dies in terms of delay, power consumption and density.






